DINO: DETR with Improved DeNoising Anchor Boxes for End-to-End Object Detection

We present DINO (\textbf{D}ETR with \textbf{I}mproved de\textbf{N}oising anch\textbf{O}r boxes), a state-of-the-art end-to-end object detector. % in this paper. DINO improves over previous DETR-like models in performance and efficiency by using a contrastive way for denoising training, a mixed query selection method for anchor initialization, and a look forward twice scheme for box prediction. DINO achieves $49.4$AP in $12$ epochs and $51.3$AP in $24$ epochs on COCO with a ResNet-50 backbone and multi-scale features, yielding a significant improvement of $\textbf{+6.0}$\textbf{AP} and $\textbf{+2.7}$\textbf{AP}, respectively, compared to DN-DETR, the previous best DETR-like model. DINO scales well in both model size and data size. Without bells and whistles, after pre-training on the Objects365 dataset with a SwinL backbone, DINO obtains the best results on both COCO \texttt{val2017} ($\textbf{63.2}$\textbf{AP}) and \texttt{test-dev} (\textbf{$\textbf{63.3}$AP}). Compared to other models on the leaderboard, DINO significantly reduces its model size and pre-training data size while achieving better results. Our code will be available at \url{https://github.com/IDEACVR/DINO}.

==> images/neg_analysis.tex <==
\begin{figure}[h]
    \includegraphics[width=\columnwidth]{images/neg_small.pdf}
    \centering
    \caption{$D^4ETR$ vs DN: the AP and AP small where AP small denotes the AP over objects whose area is below $30\times$30.}
    \label{fig:neg analysis}
    \vspace{-0.3cm}
\end{figure}

==> images/unstable_matching.tex <==
\begin{figure}[h]
    \includegraphics[width=\columnwidth]{images/vis_unstanble_compare.png}
    \centering
    \caption{Mismatch ratios of different layers for two matching methods. The terms ``post'' and ``pre'' are used for post-matching strategy and pre-matching strategy, respectively. }
    \label{fig:matching_unstable}
    % \vspace{-0.3cm}
\end{figure}

==> tables/sota_table.tex <==
\begin{table}[h]
    \centering
        \footnotesize
            \renewcommand{\arraystretch}{1.3}
    \resizebox{1.0\columnwidth}{!}{%
    \begin{tabular}{c|c|c|c|c|c|c|c|c}
        \shline
        Method & params & backbone pretrain dataset & model pretrain dataset & use mask & end-to-end &TTA& AP(val) & AP(test) \\
        \shline
        SwinL~\cite{liu2021swin} & $284$M & IN-22K-14M & O365  & \checkmark & & \checkmark& $58.0$ & $58.7$ \\
        DyHead~\cite{dai2021dynamic} & $\geq 284$M & IN-22K-14M & Unknown*  &  &  & \checkmark& $58.4$ & $60.6$ \\
        Soft Teacher+SwinL~\cite{xu2021end} & $284$M & IN-22K-14M & O365  & \checkmark & & \checkmark& $60.7$ & $61.3$ \\
        GLIP~\cite{li2021grounded} & $\geq 284$M & IN-22K-14M & FourODs~\cite{li2021grounded},GoldG+ &  & & \checkmark& $60.8$ & $61.5$\\
        Florence-CoSwin-H\cite{yuan2021florence} & $\geq 637$M & FLD-900M~\cite{yuan2021florence} &  FLD-9M~\cite{yuan2021florence} & \checkmark & & \checkmark& $62.0$ & $62.4$ \\
        SwinV2-G~\cite{liu2021swinv2} & $3.0$B & IN-22K-ext-70M~\cite{liu2021swinv2} & O365 & \checkmark & & \checkmark& $62.5$ & $63.1$\\
        \hline
        % DN-DAB-DETRv2-SwinL(Ours) & $200$M & $14$M & $1.7$M &  & \checkmark& $\textbf{63.1}$ & $\textbf{63.3}$ \\
        D$^{4}$ETR-SwinL(Ours) & $\textbf{218}$\textbf{M} & IN-22K-14M & O365 &  & \checkmark&& $\textbf{63.1}$ & $\textbf{63.2}$ \\
        D$^{4}$ETR-SwinL(Ours) & $\textbf{218}$\textbf{M} & IN-22K-14M & O365 &  & \checkmark& \checkmark& $\textbf{63.1}$ & $\textbf{63.3}$ \\
        \shline
    \end{tabular}
    }
    \vspace{0.3cm}
    \caption{Comparisons of the best detection models on MS-COCO. Similar to DETR~\cite{carion2020end}, we use the term ``end-to-end'' for the models that are free from head-drafted components like RPN and nms. The term ``use mask'' means that if the models are trained with segmentation annotations. We use the terms ``IN'',``O365'' for the ImageNet~\cite{deng2009imagenet} and Objects365~\cite{shao2019objects365} datasets, respectively. Note that ``O365'' is a subset of ``FourODs'' and ``FLD-9M''. *The DyHead did not present the details of the datasets used for model pre-training.
    }
    \label{tab:sota}
\end{table}

% \begin{table*}[h]
%     \centering
%         \footnotesize
%             \renewcommand{\arraystretch}{1.3}
%     \resizebox{1.0\columnwidth}{!}{%
%     \begin{tabular}{c|c|c|c|c|c|c|c}
%         \shline
%         Method & params & backbone data size & pretrain data size & use mask & end-to-end & AP(val) & AP(test) \\
%         \shline
%         SwinL~\cite{liu2021swin} & $284$M & $14$M & $1.7$M  & \checkmark & & $58.0$ & $58.7$ \\
%         DyHead~\cite{dai2021dynamic} & $\geq 284$M & $14$M & $\geq 1.7$M  &  &  & $58.4$ & $60.6$ \\
%         Soft Teacher+SwinL~\cite{xu2021end} & $284$M & $14$M & $1.7$M  & \checkmark & & $60.7$ & $61.3$ \\
%         GLIP~\cite{li2021grounded} & $\geq 284$M & $14$M & $22$M &  & & $60.8$ & $61.5$\\
%         Florence-CoSwin-H\cite{yuan2021florence} & $\geq 637$M & $900$M & $9$M & \checkmark & & $62.0$ & $62.4$ \\
%         SwinV2-G~\cite{liu2021swinv2} & $3.0$B & $3.5$B & $1.7$M & \checkmark & & $62.5$ & $63.1$\\
%         \hline
%         % DN-DAB-DETRv2-SwinL(Ours) & $200$M & $14$M & $1.7$M &  & \checkmark& $\textbf{63.1}$ & $\textbf{63.3}$ \\
%         D$^{4}$ETR-SwinL(Ours) & $218$M & $14$M & $1.7$M &  & \checkmark& $\textbf{63.1}$ & $\textbf{63.3}$ \\
%         \shline
%     \end{tabular}
%     }
%     \vspace{0.3cm}
%     \caption{Comparisons of the best detection models on MS-COCO. Similar to DETR~\cite{carion2020end}, we use the term ``end-to-end'' for the models that are free from head-drafted components like RPN and nms. The term ``use mask'' means that if the models are trained with segmentation annotations.
%     }
%     \label{tab:ablation}
% \end{table*}
